Active model split hybrid RANS/LES

Reliably predictive simulation of complex flows requires a level of model sophistication and robustness exceeding the capabilities of current Reynolds-averaged Navier-Stokes (RANS) models. The necessary capability can often be provided by well-resolved large eddy simulation (LES), but, for many flows of interest, such simulations are too computationally intensive to be performed routinely. In principle, hybrid RANS/LES (HRL) models capable of transitioning through arbitrary levels of modeled and resolved turbulence would ameliorate both RANS deficiencies and LES expense. However, these HRL approaches have led to a host of unique complications, in addition to those already present in RANS and LES. This work proposes a modeling approach aimed at overcoming such challenges. The approach presented here relies on splitting the turbulence model into three distinct components: two responsible for the standard subgrid model roles of either providing the unresolved stress or dissipation and a third which reduces the model length scale by creating resolved turbulence. This formulation renders blending functions unnecessary in HRL. Further, the split-model approach both reduces the physics-approximation burden on simple eddy-viscosity-based models and provides convenient flexibility in model selection. In regions where the resolution is adequate to support additional turbulence, fluctuations are generated at the smallest locally resolved scales of motion. This active forcing drives the system towards a balance between RANS and grid-resolved LES for any combination of resolution and flow while the split-model formulation prevents local disruption to the total stress. The model is demonstrated on fully-developed, incompressible channel flow [1] and the periodic hill [2], in which it is shown to produce accurate results and avoid common HRL shortcomings, such as model stress depletion.

==> anisotropy.tex <==


{\color{blue}

In practical flows of engineering interest, the combination of high
Reynolds number with complex geometries and limited computational
resources often dictates discretization using relatively high
aspect ratio (AR) cells of varying shape and rapidly varying size in
space.  In such cases, the assumptions of isotropic unresolved
turbulence in equilibrium with the large scales and isotropic LES
filtering will often be violated.  Accordingly, issues of both
turbulence and resolution anisotropy must be addressed.

In previous work, we applied a resolution-scale
anisotropy representation to the entire LES model term by introducing a
direction-dependent eddy viscosity~\cite{HaeringPhd}:
\begin{equation}
  \tau_{ij}=\nu_{jm}\partial_m\bar{u}_i+\nu_{in}\partial_n\bar{u}_j,
  \label{tau_bar}
\end{equation}
with multiple tensor eddy viscosity models having been constructed and
evaluated~\cite{year2}.  In light of the model-splitting
method (\S\ref{sec:blending_proposal}), the generalization of this
approach requires two eddy viscosity tensors.  Consistent with the
purpose of each component of the subgrid model, model anisotropy can
be divided into two main categories: turbulent stress anisotropy and
dissipation anisotropy.  Stress anisotropy describes how momentum is
transferred differently between each velocity component in the flow.
Dissipation anisotropy, on the other hand, describes the different
rates of energy transfer to unresolvable scales resulting from each
velocity component and filter direction.  The former is primarily due
to the largest scales of turbulence while the latter depends on the
smallest resolved scales.  These effects are separated in the
model-split hybridization approach, and thus, separate anisotropy models can
also be used.

Since stress anisotropies are mostly carried by the largest of
turbulent structures, it is reasonable to expect that even small
resolved turbulent kinetic energy will result in adequate total stress
anisotropy in the model-splitting approach.  This is, in fact, one of
the main reason for hybrid modeling.  An important reason for poor
RANS performance is poor representation of Reynolds stress
anisotropy \cite{laun:1975}.  If the hybrid approach is correctly
formulated, such anisotropies should be captured in regions where
sufficient resolution is provided.  In this case, scalar $\nu_t$
models should be sufficient for $\tau_{ij}^{SGRS}$.  Thus, in this initial
work, a standard $\overbar{v^2}$-$f$-based RANS model, specifically
the code-friendly version\cite{lien:2001}, is used, but any of the
standard models could be used.  Anisotropic models for $\tau_{ij}^{SGRS}$
will be explored at a later time.

As the dissipation anisotropy is responsible for different rates of
resolved energy removal in each direction, it does directly affect the
structure of the resolved turbulence near the cutoff.  
Simulations of forced, homogeneous, isotropic
turbulence with anisotropic meshes have shown that the following eddy
viscosity tensor, labeled the ``M43'' model, gives reasonable results~\cite{haer:2018}
\begin{equation}
\nu^t_{ij}=C(\mathcal{M})\la\varepsilon\ra^{1/3}\mathcal{M}^{4/3}_{ij},
\label{nu_m43}
\end{equation}
where $\la\varepsilon\ra$ was set equal to the power input by
low-wavenumber stirring and the ``constant'' is a function of the
eigenvalues of $\mathcal{M}$ found by fitting to the expected
dissipation using the expected grad-grad product,
$\la{}\partial_ku^>_i\partial_lu^>_j\ra$, assuming a $k^{-5/3}$
inertial range spectrum.  Note that the $C(\mathcal{M})$ used here corresponds to 
second-order finite volume numerics and is not the same is of that presented in 
\cite{year2} where a psuedo-spectral code was used.  The specific coefficients 
used here are given in the appendix.  When applied to varying AR cells and 
shapes, (\ref{nu_m43}) was shown to be greatly superior to Smagorinsky and nearly
equivalent to AMD \cite{roze:2015} (Fig. \ref{fig:Ek}).  This is particularly interesting
because both of these previous scalar eddy viscosity forms are expressed in 
terms of instantaneous fluctuating velocity gradients, and therefore vary greatly and 
may contribute to the mean stress as there may be non-vanishing 
correlations.  The tensor eddy viscosity~\eqref{nu_m43} however, relies on no gradient
information and does not fluctuate.  Therefore, the fluctuating gradient portion
does not contribution to the mean stress.  With the $\overbar{v^2}$-$f$ model used 
here, the required expected dissipation is set to the RANS model $\varepsilon$.
\begin{comment}
%
\begin{figure}
\begin{center}
\includegraphics[width=0.6\linewidth]{smag_m43_book.pdf}
\end{center}
\caption{Fine and coarse directional energy spectra for ($1:32:32$) AR grids and infinite $Re$ forced HIT using standard Smagorinsky and (\ref{nu_m43}).}
\label{fig:Ek}
\end{figure}
\end{comment}

\begin{comment}
 \begin{figure}[h!]
 %\begin{center}
 
 \begin{subfigure}{0.3\linewidth}{\includegraphics[width=0.3\linewidth]{figures/smag_Lbook_both.pdf} }
% \begin{subfigure}{0.1\linewidth}{\includegraphics{figures/smag_Lbook_both.pdf} }
 \caption{Smagorinsky}
 \end{subfigure}

 \begin{subfigure}{0.3\linewidth}{\includegraphics[width=0.3\linewidth]{figures/amd_Lbook_both.pdf} }
 \caption{AMD}
 \end{subfigure} 
 
 \begin{subfigure}{0.3\linewidth}{\includegraphics[width=0.3\linewidth]{figures/m43_Lbook_both.pdf} }
 \caption{M43}
 \end{subfigure}
  
 %\subfigure[M43 low k]{\includegraphics[width=0.45\linewidth]{figures/m43b_Lbook_both.pdf} \label{m43bLl}} \\
 %\end{center}
 \caption{Directional energy spectra with book cells at ratios of minimum cutoff to minimum resolved wavenumbers of $(2:1)$ to $(16:1)$ with a fixed aspect ratio of $(8:1)$, normalized by $\varepsilon^{2/3}\kappa_{min}^{-5/3}$ and equivalently filtered theoretical $k^{-5/3}$ energy spectra.}
 \label{fig:Ek}
 \end{figure}
 \end{comment}

In the model-split hybridization approach, this model form can be used for
$\tau^{SGET}$ with the necessary mean dissipation provided by the RANS
model.  This choice is used in the example in~\S\ref{sec:results}.
 

%\textcolor{red}{\emph{Move this bit elsewhere...}}
\subsection{Similarities with Existing Models}
Though the proposed hybrid structure is unique in total with particularly novel components, it does share 
qualities with existing methods and, in the case of DES, expanded on existing concepts.  The anisotropic resolution adequacy 
parameter collapses to the lengthscale comparison driving all DES methods under 
the conditions of isotropic resolution and equilibrium/isotropic turbulence.  
The DHRL method \cite{bhus:2012} similarly divides the total modeled 
stress into RANS-based and LES-based models but retains dependance 
on the total resolved velocity field for each contribution while introducing 
blending between each term based on their resulting production.   The 
dual-mesh hybrid methods of \cite{jenn:2017} explicitly solves a RANS 
and LES set of equations on disparate grids and also uses time-averaging 
to enforce consistency between the resolved and modeled fields by 
modification of the RANS stress with the average of the resolved Reynolds 
stress present in the LES equations.  Such an approach does provide 
and improved mean but it is unclear how it used to improve the turbulence 
modeling beyond the changes to mean terms.

\begin{comment} % don't talk about grid inhomogeneity b/c we don't treat it here
\subsubsection{Grid Inhomogeneity}
When convecting through coarsening grids, the rate of reduction of
resolvable scales in the streamwise direction may exceed the rate 
at which $\tau^{SGET}$ computed using the local $\mathcal{M}$ can remove energy.
%, when its response is dictated solely by the local change in $\mathcal{M}$.
That is, unresolvable
turbulence will be convected into coarser regions faster than the model can
remove it, since the critical time scale is then related to the
convective time scale, not the turbulence time scale itself.  To
avoid this behavior, a mechanism for managing the resolved turbulence
is required, but in this case, the forcing described
in~\S\ref{sec:forcing_proposal} is not appropriate.

We propose to assist the SGET model in removing energy from
the resolved scales by altering the resolution tensor.  Specifically,
a modified resolution tensor based on the mean
convective velocity and gradient of the resolution,
\begin{equation}
\mathcal{M}^*_{ij}
=
\mathcal{M}_{ij}
+
C_{\mathcal{M}}\frac{\alpha{}k_{tot}}{\varepsilon}\la{}u\ra_k\partial_k\mathcal{M}_{ij},
\label{mstar}
\end{equation}
should avoid energy pile-up at the cutoff in regions of high-speed 
flows with complex domains and grids. Where both the gradient of the resolution and the flow
direction are aligned, the effective resolution tensor $\mathcal{M}^*$
will be larger than the standard $\mathcal{M}$.  Thus, the SGET model
will remove energy more rapidly.   As proposed, (\ref{mstar}) will also reduce the the model
length scales when convecting into refining regions allowing the
energy cascade to populate the additional scales of motion.  Further,
it may be beneficial to use $\mathcal{M}^*$ in the resolution adequacy parameter (\ref{rd}) to induce active injection of fluctuations as the flow enters regions of finer resolution as opposed to once it is already there.

Both these developments will be investigated in isolation in pure LES
simulations. Thus, we propose to test and refine this approach with
LES of isotropic turbulence convecting through regions of varying
resolution.  Once the model has been developed and tested in that
context, it will be integrated with the forcing discussed
in~\S\ref{sec:forcing_proposal}, 
%which is necessary to initialize
%fluctuations in regions where little or no resolved content exists,
and tested in the hybrid formulation.
\end{comment}



}%\color




==> complete.tex <==

%HRL methods suffer from existing RANS and LES shortcomings while introducing unique 



The first main shortfall is the cause of MSD has been discussed in the previous section and 
elsewhere \cite{}.  Essentially, inconsistency in the resolved and modeled turbulence arise 
from combinations of reliance on passive self-generation of resolved turbulence in the presence 
of reduced modeled stress and the overarching hybridization strategy only affecting the model 
behavior.  Hybrid methods should not only provide the unresolved contribution to the turbulent 
stress but also govern, or at least respond to, the total turbulence stress. We propose that 
body forcing must be a component of an HRL framework and that modeled stress must only 
be reduced in response to locally resolved fluctuations.

Second, single-model unified HRL approaches based on RANS models (DES, PANS, PITM) often 
tacitly assume nonlinear source terms, which are constructed and calibrated to function in a RANS 
simulation with only mean quantities, to perform in similarly when used with fluctuating 
quantities.  Such terms are themselves models for actual scalar transport terms and use with fluctuating terms 
may generally result is spurious correlations which non-negligibly affect their mean behavior.  For 
instance, consider the model for the destruction of dissipation in $\varepsilon$ transport equation \cite{}
\begin{equation}
2\overbar{\partial_j\partial_k{}u_i\partial_j\partial_k{}u_i}\approx{}C_{\varepsilon{}2}\frac{\varepsilon^2}{k},
\end{equation}
which is used in all $k$-$\varepsilon$ based RANS models.  The model has little physical basis 
but is functional for mean flows with coefficient tuning in conjunction with other modeling 
errors.  However, expanding in Taylor series about $1/\la{}k\ra$ reveals
  \begin{equation}
 \bigg{\la}\frac{\varepsilon^2}{k}\bigg{\ra} \approx  \frac{ \langle{} \varepsilon \rangle{}^2}{\langle k \rangle}
\left( 
1
+
\frac{ \langle{} \varepsilon'^2 \rangle{} }{\langle \varepsilon \rangle^2}
+
\frac{ \langle k'^2 \rangle }{\langle k \rangle^2}
-
\frac{ \langle \varepsilon' k' \rangle }{\langle \varepsilon \rangle \langle k \rangle}
-
\frac{ \langle{} \varepsilon'^2 k' \rangle }{\langle \varepsilon \rangle^2 \langle k \rangle}
+
\frac{ \langle{} \varepsilon' k'^2 \rangle{} }{\langle \varepsilon \rangle \langle k \rangle^2}
+
\frac{ \langle{} \varepsilon'^2 k'^2 \rangle{} }{\langle \varepsilon \rangle^2 \langle k \rangle^2}
\right)
\end{equation}
}
while the behavior of mixed terms is not obvious, auto-correlations are clearly positive definite 
for any fluctuations.  Thus, the mean destruction of dissipation becomes a direct, and complicated, 
function of the amount of resolved turbulence.  Even the standard RANS production term, 
$\mathcal{P}_k=2\nu_t\la{}S\ra^2$, is itself a model and will exhibit spurious correlations, depending 
on the particular RANS model used to determine $\nu_t$, when used with fluctuations quantities.  Thus, 
all nonlinear terms in transport models must either have coefficients which depend on the level of 
resolved turbulence or must only be constructed with expected value parameters.

Third, HRL requires the model to provide both non-negligible 
contributions to the unresolved stress and the transfer of energy from resolved scales of 
motion to the subgrid.  However, when used in an LES, simple scalar eddy viscosities typically 
only provide the latter while being significantly under predictive of the former \cite{}.  In 
such cases, \emph{i.e.} ``well-resolved'' LES, the majority of turbulence stress is resolved 
and errors in the subgrid are tolerable.  On the opposite end of the resolved spectrum, even 
for flows where an eddy viscosity model provides a good approximation of the total turbulent 
stress for RANS, there is no reason to expect the same model to provide the correct energy transfer 
for the resolved fluctuations 







==> devc.tex <==

Next, we examine the spatially developing characteristics of the
hybrid method by extending the length of the channel to $10\pi$ and
using a RANS inlet condition with convective outflow.  Thus, this test
case is more representative of typical applications.  The grid spacings
in plus units has been coarsened to $\Delta^+\approx450$ in the span 
and streamwise directions.  The results are summarized in Figures~\ref{fig:spatial}.
%
\begin{figure}[htp!]
\begin{center}
\subfigure[Plane averaged $\bar{u}_x$ and $\alpha$]{
\includegraphics[width=0.45\linewidth]{figures/spatial_ux.pdf}
\label{s_mux}
}
%
\subfigure[Turbulent kinetic energy]{
\includegraphics[width=0.45\linewidth]{figures/spatial_tke.pdf}
\label{s_mtke}
}
\begin{overpic}
[trim={0.2cm 29.2cm 0.2cm 29.2cm},clip=true,width=0.95\linewidth]{figures/long_chan_ux.png}
\put(10.0,1.0){\color{lblue}\rule{1pt}{27.0pt}}
\put(30.0,1.0){\color{yellow}\rule{1pt}{27.0pt}}
\put(50.0,1.0){\color{blue}\rule{1pt}{27.0pt}}
\put(70.0,1.0){\color{red}\rule{1pt}{27.0pt}}
\put(90.0,1.0){\color{green2}\rule{1pt}{27.0pt}}
\put(-2.6,2.6){\color{black}\rotatebox{90}{$\overbar{u_x}$}}
\end{overpic}
%
\begin{overpic}
[trim={0.2cm 29.2cm 0.2cm 29.2cm},clip=true,width=0.95\linewidth]{figures/long_chan_rm.png}
\put(-3.0,1.5){\color{black}\rotatebox{90}{$\la{}r_\mathcal{M}\ra$}}
\end{overpic}
%
\end{center}
\caption{Normalized mean streamwise velocity for channel flow at $Re_\tau\approx5200$ with overlaid level of resolved turbulence (a) and TKE (b).  Plane-averaged at positions:  \textcolor{lblue}{---}$\pi$, \textcolor{yellow}{---} $3\pi$, \textcolor{blue}{---} $5\pi$, \textcolor{red}{---} $7\pi$, and \textcolor{green2}{---} $9\pi$ as indicated in the contour plot of $\overbar{u_x}$.  Both $\overbar{u_x}$ and $\la{}r_\mathcal{M}\ra$ use the same colormap as in Fig. \ref{fig:rd_ux}}
\label{fig:spatial}
\end{figure}

Again, for all spatial locations and levels of resolved turbulence,
the expected logarithmic profile in the mean streamwise velocity is
attained (Fig. \ref{s_mux}).  A very minor deviation is observed at
the $7\pi$ location.  Resolved turbulence develops more gradually in
the core of the channel in comparison to around $y^+\approx1000$.
This is likely due to the magnitude of the forcing scaling with the
local TKE and time scale (Eq. \ref{Ftar}).  The under-utilized
resolution is apparent in accompanying $\la{}r_\mathcal{M}\ra$ contour
plot where the grid-resolved LES ``front'' has not extended to the
channel center by the outlet. Naturally, it is highly desirable for
the model to transition from RANS to grid-resolved LES with as little
time and space as possible.  Therefore, improving slow-core
development is another avenue for improving future forcing
formulations.  Contrary to results in the temporally developing case
(Fig.~\ref{mtke}), the TKE from both the RANS model and accounting for
the contribution from the resolved, field exceeds the DNS value in the
center of the channel (Fig.~\ref{s_mtke}).  The reason for this
inconsistency is not apparent though it does not seem to corrupt the
mean flow.




==> intro_forcing.tex <==



By themselves, typical HRL methods rely on natural flow instabilities to self-generate resolved 
fluctuations in regions where the modeled stress is reduced.  Therefore, by construction, 
they will all exhibit regions of modeled-stress-depletion (MSD) \cite{} as it is only through 
the depleted total stress that the desired instabilities can develop.  This is assuming the 
mean shear is large enough to be unstable.  It is entirely possible that turbulent regions 
of flow exist where reducing the model to zero will not result in the development of resolved 
fluctuations \cite{Davidson, 2006}.  Through multiple simulations by separate researchers 
with disparate models, the necessity of some type of active forcing in hybrid simulations 
has become abundantly clear \cite{spal:XXXX,ment:2010,?}.  Explicitly introducing resolved 
fluctuations, at a rate so that the additional stress is equivalent to the rate of reduced model 
stress, is the only way to prevent regions of MSD.  Common issues such as log-layer 
mismatch, reduced body forces, premature flow separation, and delayed flow reattachment 
will otherwise persist in HRL.

Existing forcing methods have typically addressed this issue by generating 
fluctuations only at a prescribed LES inlet \cite{Shur2014,Spalart2017,tabor:2010,patil:2012}.  In addition 
to requiring specification of the distinct LES region and entire spectrum of locally 
resolved synthetic turbulent scales and intensities, the LES inlet location must be 
sufficiently upstream of the actual feature of interest so that the artificial inflow 
condition can ``heal'' to a realistic state.  Body forcing may be thought of as a 
method to introduce synthetic turbulence at a ``healing'' rate so that, through the 
entire forced region, the flow maintains a realistic state.  In this way, none of the 
simulated domain and associated computational cost is sacrificed allowing the entire 
simulated solution to yield useful information.  

In channel flow, Piomelli \emph{et.al.} \cite{piom:2003} found that introducing a region of wide 
tuned stochastic forcing in a thin region along the RANS/LES interface region eliminates log-layer 
mismatch in fully developed channel flow using HRL.  While being problem 
specific and difficult to implement in general, this numerical test revealed bands of 
body forcing in regions of transition from RANS to LES can solve problems related to MSD.  
The notion of adding user-specified regional body forcing was further explored by Menter \emph{et.al.} 
in the SAS-F model \cite{ment:2010}.  In their work, a wide spectrum of velocity was 
produced using the random flow generator (RFG) \cite{Batt:2004} over used to construct 
an acceleration term with the discrete timestep.  The unique aspect of their construction is that the 
basic SAS model form allows for the model to detect the added fluctuations and 
naturally respond by lowering the internal model length scale and corresponding 
eddy viscosity.  Even so, channel flow results still exhibited log layer mismatch.

As presented in \S\ref{}, a body forcing method is presented without explicit time step 
dependance and being endowed with a structure that is restricted to be only at the scale 
of the smallest locally resolved turbulence thereby reducing the potential corruption of 
existing, and presumably realistic.  Further, no user specification forcing-regions are 
necessary.


\begin{comment}
based on the variable length scale TG field and subgrid velocity 
scale rather than relying on generation of a wide spectrum of fluctuations using the 
Random Flow Generator method \cite{krai:1969,batt:2004}.  By restricting the forcing 
structure to be only at the scale of the smallest locally resolved turbulence, existing 
larger, and presumably realistic, structures are not corrupted.
\end{comment}



==> intro_hybrid.tex <==


An excellent review of HRL methods is presented by Fr\"{o}lich and von Terzi \cite{froh:2008} 
while a specific review of the most ubiquitous method of detached eddy simulation (DES) is 
provided by Spalart \cite{spal:2009} and more recently by Gritskevich \emph{et.al.} 
\cite{Menter:2017} for the particular combination of DES with wall functions.  In general, HRL 
methods function either by reducing the model with some specified function \cite{spez}, 
carrying distinct RANS and LES models with some blending of the respective modeled stress 
terms \cite{fan:2004}, or by carrying a single model which internally transitions between RANS 
and LES-like modes of operation \cite{des,pans,pitm}.  For all methods, the model transition 
may be in response to the local model/flow parameters and a measure of the grid size (``unified'') 
\cite{} or specified \emph{ab-initio} (``interfaced'') \cite{}.  Transition from RANS to LES in unified 
methods tend to rely on \emph{ad-hoc} functions requiring tuning for specific flows (model reduction 
factor in FSM\cite{}, delaying funciton in DDES\cite{}, for example).  All these methods are based on 
the basic Boussinesq assumption with the modeled stress being approximated by some eddy viscosity 
operating on the resolved strain rate tensor.  

Since the aforementioned review, additional methods have emerged.  Of particular 
interest to the development presented here are the dynamic hybrid RANS/LES (DHRL) \cite{bush:2012,walt:2012} 
and the Jenny group \cite{xiao:2017} approaches.  Falling in the category of blended distinct RANS and 
LES models, the DHRL method makes the small, yet significant, deviation of allowing 
each model to act on different portions of the resolved strain rate tensor.  In particular, 
the RANS eddy viscosity acts only on the mean strain rate while the LES eddy viscosity acts on 
the entire resolved strain.  Additionally, all quantities entering the RANS model are mean values.  
Such modifications acknowledge that models developed for RANS 
are not appropriate for use with fluctuating quantities while SGS models, developed for LES, 
are\todo{fix passive}.  The Jenny group dual-mesh approach explores the extreme of interfaced methods (``segregated'') by 
coupling distinct LES and RANS simulations through the use of additional terms which enforce 
some consistency of the mean of resolved velocity evolution and the Reynolds averaged TKE evolution as approximated by 
causal time averaging.  This basic concept explicitly makes use of the fact that the RANS equations 
should remain valid in multiscale methods regardless of the level of resolved or modeled 
turbulence.

As presented in \S\ref{} and discussed in \S\ref{}, the proposed model uses elements from 
standard DES, DHRL, and the Jenny group method while also eliminating the distinction 
between reduced, blended, and hybridized single-model HRL methods.


==> intro_orig.tex <==


In the absence of revolutions in either computational capabilities or the accuracy and 
generality of RANS models, flexible turbulence modeling methods allowing for mixed 
degrees of modeled and resolved turbulence will remain a necessity until the turn 
of the century \cite{spal:2000}.  Driven not only by well-known inadequacies of RANS in 
the presence of complex flow features such as separation, reattachment, or generally 
any flow with a three-dimensional mean \cite{wilcox:2001}, multiscale methods are also needed 
to provide additional information, in a computationally feasible manner, such as unsteady 
fluid-structure interactions to predict structural vibrations \cite{} or \textcolor{red}{something about 
ignition?}.  In response to these requirements, a myriad of multiscale turbulence modeling 
techniques have been proposed and developed \cite{}.  Three main categories  
have emerged, physics-free numerically stabilized variational multiscale 
(VMS)\cite{}, wall-modeled large eddy simulation (WMLES)\cite{}, and hybrid RANS/LES 
(HRL) \cite{}.  The latter has garnered widespread attention largely due to the formal 
similarities in the RANS and filtered Navier-Stokes equations \cite{} leading to the 
attractive, yet perhaps misleading, prospect of simply blending between respective 
models in a manner amenable to existing CFD code structure.  Despite extensive effort, a truly robust HRL approach remains elusive.  
Amongst others, reasons for this include a reliance on passive generation of resolved turbulence 
in the presence of reduced modeled stress and the over-burdening of simple scalar 
eddy viscosity models with providing both significant portions of the unresolved stress and 
modeling the transfer of energy from the resolved fluctuations to the subgrid.  Here, 
we propose an HRL method which directly addresses these common issues.

\textcolor{red}{\emph{This next paragraph gets into some controversial territory, need to back it up more...}}\\
Often, there exists a great deal of overlap between VMS, WMLES, and HRL.  For 
instance, HRL where the RANS model is only active near the wall \cite{spal:1996} may 
be considered a WMLES.  However, the true potential power of WMLES lies in obviating 
log-layer resolution with newly emerging methods such as slip-length models \cite{}.  Were such an approach 
made to be robust for complex flows, WMLES would be the clear ``winner'' for 
wall-bounded flows.  However, until such an advance is made, HRL methods, with 
RANS-quality near wall resolutions, are the most widely applicable approaches.  
Further common overlap is present when any multiscale turbulence method makes use of 
numerical dissipation, most notably upwinding of the convective term, as these are essentially 
mixing VMS aspects with the supposedly immaculate\textcolor{red}{(change word)} approach \cite{giri:1996}.  As previously 
stated, the method proposed here is distinctly in the family of HRL and we restrict our 
further discussion accordingly.




==> wmh.tex <==


%\subsubsection{Wall-mounted hump}
The final incompressible test case is the 2D-hump in cross-flow of Greenblatt 
et al.~\cite{green:2006}.  The data show smooth-wall reattachment, 
which current RANS and hybrid methods often fail to predict correctly,
making this an excellent case for hybrid model validation.  However, contrary 
to the periodic hill case, there is a long smooth run-up to the separation point. 
This is significant in that the large turbulent structure in the outer portion of the 
boundary layer are not ``jostled'' into the separated shear layer.  Therefore, 
shear layer breakup, which is necessary to get the correct reattachment and 
recirculation region, is mediated by the very small near-wall structures at the 
separation location.  The seemingly small change in hump vs hill geometry 
necessitates resolving smaller turbulence much closer to the wall.  The 
resulting meshing constraint is further exasperated by the need for the span 
of the domain to be large enough so that large spanwise vortices in the 
recirculation region are not overly stable due to correlation of the structures 
throughout the entirety of the span.  As discussed in~\S\ref{sec:tams_motivation}, 
this case was instrumental in revealing flaws in previous hybrid methods 
developed during this project.  Unfortunately, the severity of both the local 
meshing and simulation domain requirements were not fully appreciated 
until recently.  The final simulation is yet to be performed.  We present here 
two intermediary simulations which support the aforementioned conclusions.

The computational domain is a truncated version of the experimental
wind tunnel with the region upstream of the measured mean velocity
profiles at $x/c=-2.14$ being discarded (Fig. \ref{chan}).  RANS
simulations of flow over a flat plat at the identical $Re$ are
performed using the $\overbar{v^2}$-$f$ \cite{lien:2001} model to
generate inlet boundary conditions for model scalars by matching the
outer region of experimental mean velocity profile (Fig. \ref{chan}c).
A slip boundary condition is prescribed at the top of the domain, and
the bottom is a no-slip wall.  The downstream boundary uses a mass
conserving outflow boundary condition, and the streamwise direction is
periodic.

Grid details are summarized as follows.  The wall normal spacing at
the wall is $\delta_{\bot}=2.5\times10^{-5}c$ ($<1y^+$ at inlet).  The
wall tangent spacing at the hump top upstream of the separation region
is $\delta_{\Vert}^\mathcal{H}=2.5\times10^{-3}c$ (Fig. \ref{chan}c),
while the wall tangent spacing at the separation point is
$\delta_{\Vert}^\mathcal{S}=1\times10^{-3}c$.  The inlet streamwise
spacing is $0.1c$.  Additionally, in the thin band
within approximately $0.05c$ of the wall, the wall normal spacing is
restricted to a maximum of $\delta_{\bot}=1\times10^{-3}c$.  Outside
this band, the wall normal spacing is grown by $10\%$ in each wall
normal step.  The ``focus'' region of $0.5c$ in the streamwise
direction aft of the hump is restricted to a maximum of
$\delta_{sep}=1\times10^{-3}c$ in the spanwise-normal plane.  
Two spans and spanwise gridding are presented here, the ``short'' 
span is $0.2c$ with $\delta_z=4\times{}10^{-3}$ while the ``long'' 
span is $0.5c$ with $\delta_z=1\times{}10^{-2}$.  Further, to ease 
the resolution requirements, $C_r$ in (\ref{rd}) is reduced to 0.5 
from 1.0.  This reduction was tested in the channel and found to 
introduce only minor disturbance to the mean velocity profile. 

The result is a grid typical of engineering studies containing highly
anisotropic cells in regions of interest.  For instance, the wall normal 
to span spacing ratio varies by three orders-of-magnitude.  The
total cell counts for the meshes for both span domains are $8.6M$.  
The inlet momentum thickness is $\approx{}9\times10^{-3}c$ 
($Re_\theta\approx7300$) which grows to $\approx{}6\times10^{-2}c$ 
at the top of the hump ($x/c=0.51$).


\begin{figure}[ht]
\begin{center}
\subfigure[Domain]{\includegraphics[width=0.87\linewidth]{figures/channel2.pdf}}\\
\subfigure[Separation Region]{\includegraphics[width=0.35\linewidth]{figures/grid.png}}
\subfigure[Inlet velocity]{\includegraphics[width=0.35\linewidth]{figures/wmh_inlet_velocity.pdf}}
\end{center}
\caption{Channel domain (a)\protect\footnotemark for the 2D hump in cross flow simulations 
with close up (b) of the separation region and (c) experimental and matched flat plate 
simulation inlet profile. The channel ceiling is offset over the hump in an attempt to account for 
blockage effects on side hump posts not directly simulated.  This feature is maintained 
from NASA domains while the grid itself is reconstructed.}
\label{chan}
\end{figure}
%\end{comment}

\footnotetext{Reproduced from the NASA Turbulence 
Modeling Resources (available: http://turbmodels.larc.nasa.gov/)} 

Results are shown in Figure~\ref{fig:tams_hump_flow} and~\ref{fig:tams_hump_cpcf}.
%
\begin{figure}[htp!]
\begin{center}
\subfigure[]{
\includegraphics[trim={0.2cm 9.25cm 0.2cm 10cm},clip=true,width=0.48\linewidth]{rans_swvort.png}
\put(-215,45){\textcolor{white}{\small{(a) RANS $\omega_z$}}}}
%
\subfigure[]{
\begin{overpic}
[trim={0.2cm 9.25cm 0.2cm 10cm},clip=true,width=0.48\linewidth]{rans_uxave.png}
\put(79,14){\color{black}\vector(0,-1){5}}
\end{overpic}
\put(-215,45){\textcolor{black}{\small{(b) RANS $\la{}u_x\ra$}}}}
%
\subfigure[]{
\includegraphics[trim={0.3cm 19.25cm 5cm 23cm},clip=true,width=0.48\linewidth]{wmh_swvort_0p2c.png}
\put(-215,45){\textcolor{white}{\small{(c) 0.2c $\omega_z$}}}}
%
\subfigure[]{
\begin{overpic}
[trim={2.0cm 10.0cm 5cm 32.4cm},clip=true,width=0.48\linewidth]{wmh_uxave_0p2c.png}
\put(86,11.0){\color{white}\vector(0,-1){5}}
\end{overpic}
\put(-215,45){\textcolor{white}{\small{(d) 0.2c $\la{}u_x\ra$}}}}
%
\subfigure[]{
\includegraphics[trim={0.3cm 19.25cm 5cm 23cm},clip=true,width=0.48\linewidth]{wmh_swvort_0p5c.png}
\put(-215,45){\textcolor{white}{\small{(e) 0.5c $\omega_z$}}}}
%
\subfigure[]{
\begin{overpic}
[trim={2.0cm 10.0cm 5cm 32.4cm},clip=true,width=0.48\linewidth]{wmh_uxave_0p5c.png}
\put(88,8.5){\color{white}\vector(0,-1){5}}
\end{overpic}
\put(-215,45){\textcolor{white}{\small{(f) 0.5c $\la{}u_x\ra$}}}}
%
\subfigure[]{
\includegraphics[width=0.48\linewidth]{exp_uave2R.png}
\put(-45,17){\textcolor{white}{\small{(i) PIV}}}}
\end{center}
\caption{Results for two hybrid model domains compared to $\overline{v^2}$-$f$ RANS, and
  experiment: Instantaneous spanwise vorticity (a,c,e) and mean streamwise velocity 
  (b,d,f,g).  The arrows indicate approximate reattachment location.  Note that the hybrid plots have 
  a different x-scale than the original RANS results.}
\label{fig:tams_hump_flow}
\end{figure}
\todo{Replace DDES with TAMS}
%
%
\begin{figure}[htp!]
\begin{center}
\subfigure[$C_p$]{
\includegraphics[trim={2cm 0cm 2.5cm 0cm},clip=true,width=0.45\linewidth]{cp_2span.pdf}}
%
\subfigure[$C_f$]{
\includegraphics[trim={2cm 0cm 2.5cm 0cm},clip=true,width=0.465\linewidth]{cf_2span.pdf}}
\end{center}
\caption{TAMS results for the NASA wall-mounted hump flow, compared to
  $\overline{v^2}$-$f$ RANS and DDES: pressure coefficient (left)
  and skin friction coefficient (right).}
\label{fig:tams_hump_cpcf}
\end{figure}
\todo{Replace with TAMS results}
%
Before discussing results, we must stress that both simulations should 
be run for a longer period of time.  While the $0.5c$ span case has 
been run for $5$ hump convective times, the $0.2c$ span case has only 
been run for $3$, \emph{i.e.} not even a full flow-through.   Even so, some 
important information is revealed from the current state of the simulations.  
Instantaneous spanwise vorticity and the time-averaged streamwise 
velocity according to (\ref{ave}) are presented in \ref{fig:tams_hump_flow}.   
Figure \ref{fig:tams_hump_cpcf} shows coefficients of pressure and 
friction for both spans in comparison with both RANS and the experimental 
values.  Both $C_p$ and $C_f$ are averaged with a static time interval of 
$2T_{conv}$ and then averaged over the span.  

First, the TAMS simulations do an excellent job of predicting $C_p$.  Both spans 
correct the small deficit on the hump top and the recovery pressure in recirculation 
region (Fig. \ref{fig:tams_hump_cpcf} a).  The wider span case provides a slightly 
better $C_p$ just after the flow separation.  However, the TAMS simulations 
capture the correct separation point whereas RANS slightly delays this as seen 
by the $C_p$ being elevated relative to the experiments.  Turning to $C_f$ 
(Fig. \ref{fig:tams_hump_cpcf} b) we see how both spans nearly exactly predicts 
the reattachment location as shown by crossing the $C_f=0$ line at the location 
as from an interpolated value from the experiments.  This is reinforced by the 
single-plane and shorter time averaged streamwise velocity contours in Fig. 
\ref{fig:tams_hump_flow} d and f.  While both TAMS cases 
greatly improve the recovery $C_f$, the $0.5c$ span does a better job than the 
$0.2c$.  However, the $0.5c$ span shows an excessive dip $C_f$ in the recirculation 
region which is improved upon in the $0.2c$ case.  We believe this improvement 
is due to the increased spanwise resolution in the thin span case 
which yields smaller resolved turbulent structure prior to separation leading to 
destabilization of large-scale recirculation structures.  However, as the $0.2c$ span 
case must be run for a longer period, this conclusion is tentative.  It also appears as 
if the $0.2c$ span more accurately captures the early hump $C_f$ around $x/c=0.2$ 
while the $0.5c$ span more favorably predicts the hump top $C_f$ at about 
$x/c=0.5$. 

While these results are clearly preliminary, it is important to emphasize that the 
reattachment length is now correctly predicted without any stress-depletion 
issues.  This is a strong indication that the model-split $\alpha$ scaling along 
with active forcing introduced here correctly models momentum transfer with 
varying levels of resolved turbulence.  It seems likely that both the wide span and 
finer spanwise resolution of the $0.2c$ case are necessary for the wall-mounted 
hump.










 


